Multi-agent Reinforcement Learning with Graph Q-Networks for Antenna Tuning

Future generations of mobile networks are expected to contain more and more antennas with growing complexity and more parameters. Optimizing these parameters is necessary for ensuring the good performance of the network. The scale of mobile networks makes it challenging to optimize antenna parameters using manual intervention or hand-engineered strategies. Reinforcement learning is a promising technique to address this challenge but existing methods often use local optimizations to scale to large network deployments. We propose a new multi-agent reinforcement learning algorithm to optimize mobile network configurations globally. By using a value decomposition approach, our algorithm can be trained from a global reward function instead of relying on an ad-hoc decomposition of the network performance across the different cells. The algorithm uses a graph neural network architecture which generalizes to different network topologies and learns coordination behaviors. We empirically demonstrate the performance of the algorithm on an antenna tilt tuning problem and a joint tilt and power control problem in a simulated environment.

==> GQN Paper/evaluation_avg_sinr_short.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dodgerblue0130240}{RGB}{0,130,240}

\begin{groupplot}[group style={group size=2 by 1,vertical sep=2.2cm}, width=0.5\columnwidth, height=3cm]
\nextgroupplot[
tick align=outside,
tick pos=left,
title style={align=left},
title={hexagonal training \\ hexagonal evaluation},
unbounded coords=jump,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={GQN,GQN-GAT,DQN,GAQ,H},
x tick label style={rotate=45, anchor=north east, inner sep=0mm},
y grid style={darkgray176},
ylabel={Average SINR (dB)},
ymin=11.8712364860283, ymax=16.1040258501573,
ytick style={color=black}
]

table{%
x  y  draw  fill
0 15.2123838276273 0,130,240 0,130,240
1 15.6683761327389 0,130,240 0,130,240
2 14.6257836637029 0,130,240 0,130,240
3 14.9621204331694 0,130,240 0,130,240
4 12.314558025762 0,130,240 0,130,240
};
\addplot [only marks, mark size=1pt,mark=*, line width=1.08pt, dodgerblue0130240]
table {%
0 15.2123838276273
1 15.6683761327389
2 14.6257836637029
3 14.9621204331694
4 12.314558025762
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
0 14.4633371385209
0 15.6787333835573
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
1 15.5383183186699
1 15.911626333606
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
2 14.1652532386594
2 14.8982876198943
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
3 14.6838843464045
3 15.5116990049138
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
4 12.0636360025796
4 12.5584725724441
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title style={align=left},
title={random training \\ hexagonal evaluation},
unbounded coords=jump,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={GQN,GQN-GAT,DQN,GAQ,H},
x tick label style={rotate=45, anchor=north east, inner sep=0mm},
y grid style={darkgray176},
% ylabel={Average SINR (dB)},
ymin=11.9134688578056, ymax=15.044383670695,
ytick style={color=black}
]
% \addplot [
%   only marks,
%   scatter,
%   scatter/@post marker code/.code={%
%   \endscope
% },
%   scatter/@pre marker code/.code={%
%   \expanded{%
%   \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
%   \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
%   }%
%   \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
% },
%   visualization depends on={value \thisrow{draw} \as \drawcolor},
%   visualization depends on={value \thisrow{fill} \as \fillcolor}
% ]
table{%
x  y  draw  fill
0 13.8998679475545 0,130,240 0,130,240
1 14.5202266488269 0,130,240 0,130,240
2 12.7471026397811 0,130,240 0,130,240
3 13.246662925662 0,130,240 0,130,240
4 12.314558025762 0,130,240 0,130,240
};
\addplot [only marks, mark size=1pt,mark=*, line width=1.08pt, dodgerblue0130240]
table {%
0 13.8998679475545
1 14.5202266488269
2 12.7471026397811
3 13.246662925662
4 12.314558025762
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
0 13.6514784774299
0 14.2640713587606
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
1 14.1219356461126
1 14.9020693610182
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
2 12.4445118843485
2 12.9143744870467
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
3 12.8077595972763
3 13.5733008337825
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
4 12.0557831674824
4 12.5667927648893
};

\end{groupplot}

\end{tikzpicture}


==> GQN Paper/submitted_8pages_version.tex/evaluation_avg_sinr.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dodgerblue0130240}{RGB}{0,130,240}

\begin{groupplot}[group style={group size=2 by 2,vertical sep=2.2cm}, width=0.5\columnwidth, height=3cm]
\nextgroupplot[
tick align=outside,
tick pos=left,
title style={align=left},
title={hexagonal training \\ hexagonal evaluation},
unbounded coords=jump,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={GQN,GQN-GAT,DQN,GAQ,H},
x tick label style={rotate=45, anchor=north east, inner sep=0mm},
y grid style={darkgray176},
ylabel={Average SINR (dB)},
ymin=11.8712364860283, ymax=16.1040258501573,
ytick style={color=black}
]
% \addplot [
%   mark=*,
%   only marks,
%   scatter,
%   scatter/@post marker code/.code={%
%   \endscope
% },
%   scatter/@pre marker code/.code={%
%   \expanded{%
%   \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
%   \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
%   }%
%   \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
% },
%   visualization depends on={value \thisrow{draw} \as \drawcolor},
%   visualization depends on={value \thisrow{fill} \as \fillcolor}
% ]
table{%
x  y  draw  fill
0 15.2123838276273 0,130,240 0,130,240
1 15.6683761327389 0,130,240 0,130,240
2 14.6257836637029 0,130,240 0,130,240
3 14.9621204331694 0,130,240 0,130,240
4 12.314558025762 0,130,240 0,130,240
};
\addplot [only marks, mark size=1pt,mark=*, line width=1.08pt, dodgerblue0130240]
table {%
0 15.2123838276273
1 15.6683761327389
2 14.6257836637029
3 14.9621204331694
4 12.314558025762
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
0 14.4633371385209
0 15.6787333835573
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
1 15.5383183186699
1 15.911626333606
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
2 14.1652532386594
2 14.8982876198943
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
3 14.6838843464045
3 15.5116990049138
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
4 12.0636360025796
4 12.5584725724441
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title style={align=left},
title={hexagonal training \\ random evaluation},
unbounded coords=jump,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={GQN,GQN-GAT,DQN,GAQ,H},
x tick label style={rotate=45, anchor=north east, inner sep=0mm},
y grid style={darkgray176},
ymin=13.3812053999202, ymax=14.9102679285393,
ytick style={color=black}
]
% \addplot [
%   mark=*,
%   only marks,
%   scatter,
%   scatter/@post marker code/.code={%
%   \endscope
% },
%   scatter/@pre marker code/.code={%
%   \expanded{%
%   \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
%   \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
%   }%
%   \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
% },
%   visualization depends on={value \thisrow{draw} \as \drawcolor},
%   visualization depends on={value \thisrow{fill} \as \fillcolor}
% ]
table{%
x  y  draw  fill
0 14.3617878195756 0,130,240 0,130,240
1 14.5672959944874 0,130,240 0,130,240
2 13.9061944671223 0,130,240 0,130,240
3 14.0579773818793 0,130,240 0,130,240
4 13.8892051755826 0,130,240 0,130,240
};
\addplot [only marks, mark size=1pt,mark=*, line width=1.08pt, dodgerblue0130240]
table {%
0 14.3617878195756
1 14.5672959944874
2 13.9061944671223
3 14.0579773818793
4 13.8892051755826
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
0 13.6304828132361
0 14.8407650863294
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
1 14.3741246174767
1 14.6665155851318
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
2 13.4507082421302
2 14.2400036315969
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
3 13.8187777202919
3 14.2905632371882
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
4 13.8348674721875
4 13.9176831068446
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title style={align=left},
title={random training \\ hexagonal evaluation},
unbounded coords=jump,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={GQN,GQN-GAT,DQN,GAQ,H},
x tick label style={rotate=45, anchor=north east, inner sep=0mm},
y grid style={darkgray176},
ylabel={Average SINR (dB)},
ymin=11.9134688578056, ymax=15.044383670695,
ytick style={color=black}
]
% \addplot [
%   only marks,
%   scatter,
%   scatter/@post marker code/.code={%
%   \endscope
% },
%   scatter/@pre marker code/.code={%
%   \expanded{%
%   \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
%   \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
%   }%
%   \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
% },
%   visualization depends on={value \thisrow{draw} \as \drawcolor},
%   visualization depends on={value \thisrow{fill} \as \fillcolor}
% ]
table{%
x  y  draw  fill
0 13.8998679475545 0,130,240 0,130,240
1 14.5202266488269 0,130,240 0,130,240
2 12.7471026397811 0,130,240 0,130,240
3 13.246662925662 0,130,240 0,130,240
4 12.314558025762 0,130,240 0,130,240
};
\addplot [only marks, mark size=1pt,mark=*, line width=1.08pt, dodgerblue0130240]
table {%
0 13.8998679475545
1 14.5202266488269
2 12.7471026397811
3 13.246662925662
4 12.314558025762
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
0 13.6514784774299
0 14.2640713587606
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
1 14.1219356461126
1 14.9020693610182
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
2 12.4445118843485
2 12.9143744870467
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
3 12.8077595972763
3 13.5733008337825
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
4 12.0557831674824
4 12.5667927648893
};


\nextgroupplot[
tick align=outside,
tick pos=left,
title style={align=left},
title={random training \\ random evaluation},
unbounded coords=jump,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={GQN,GQN-GAT,DQN,GAQ,H},
x tick label style={rotate=45, anchor=north east, inner sep=0mm},
y grid style={darkgray176},
ymin=12.4980469653835, ymax=14.6419089167212,
ytick style={color=black}
]
% \addplot [
%   mark=*,
%   only marks,
%   scatter,
%   scatter/@post marker code/.code={%
%   \endscope
% },
%   scatter/@pre marker code/.code={%
%   \expanded{%
%   \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
%   \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
%   }%
%   \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
% },
%   visualization depends on={value \thisrow{draw} \as \drawcolor},
%   visualization depends on={value \thisrow{fill} \as \fillcolor}
% ]
table{%
x  y  draw  fill
0 14.1339137367683 0,130,240 0,130,240
1 14.1588300117923 0,130,240 0,130,240
2 13.2511196236829 0,130,240 0,130,240
3 13.5645249401368 0,130,240 0,130,240
4 13.8892051755826 0,130,240 0,130,240
};
\addplot [only marks, mark size=1pt,mark=*, line width=1.08pt, dodgerblue0130240]
table {%
0 14.1339137367683
1 14.1588300117923
2 13.2511196236829
3 13.5645249401368
4 13.8892051755826
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
0 13.7336685067439
0 14.5444606462059
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
1 14.0072339985084
1 14.3512995616537
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
2 12.5954952358988
2 14.0937314262046
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
3 12.6867197183605
3 14.5345217022371
};
\addplot [line width=1.08pt, dodgerblue0130240]
table {%
4 13.8348674721875
4 13.9176831068446
};
\end{groupplot}

\end{tikzpicture}

